Efficient Computation of $N$-point Correlation Functions in $D$ Dimensions

We present efficient algorithms for computing the $N$-point correlation functions (NPCFs) of random fields in arbitrary $D$-dimensional homogeneous and isotropic spaces. Such statistics appear throughout the physical sciences, and provide a natural tool to describe stochastic processes. algorithms for computing the NPCF components have $\mathcal{O}(n^N)$ complexity (for a data set containing $n$ particles); their application is thus computationally infeasible unless $N$ is small. By projecting the statistic onto a suitably-defined angular basis, we show that the estimators can be written in a separable form, with complexity $\mathcal{O}(n^2)$, or $\mathcal{O}(n_{\rm g}\log n_{\rm g})$ if evaluated using a Fast Fourier Transform on a grid of size $n_{\rm g}$. Our decomposition is built upon the $D$-dimensional hyperspherical harmonics; these form a complete basis on the $(D-1)$-sphere and are intrinsically related to angular momentum operators. Concatenation of $(N-1)$ such harmonics gives states of definite combined angular momentum, forming a natural separable basis for the NPCF. As $N$ and $D$ grow, the number of basis components quickly becomes large, providing a practical limitation to this (and all other) approaches: however, the dimensionality is greatly reduced in the presence of symmetries; for example, isotropic correlation functions require only states of zero combined angular momentum. We provide a \textsc{Julia} package implementing our estimators, and show how they can be applied to a variety of scenarios within cosmology and fluid dynamics. The efficiency of such estimators will allow higher-order correlators to become a standard tool in the analysis of random fields.

==> old.tex <==

\section{Methods}
\subsection{Definitions}
Consider a random field $\delta:\mathbb{Q}^N\to\mathbb{C}$ where $\mathbb{Q}^D$ is some $D$-dimensional manifold equipped with a Riemannian manifold. We define the $N$-point correlation function (hereafter NPCF) of $\delta$ as
\beq\label{eq: NPCF-statistic}
    \zeta(\vr^1,\ldots,\vr^{N-1};
    \vs) = \av{\delta(\vs+\vr^1)\ldots\delta(\vs+\vr^{N-1})}
\eeq
where $\av{\ldots}$ indicates an average over realizations of $\delta$ and $\vr\in \mathbb{Q}^N$ is a coordinate chart. Assuming the space to be statistically homogeneous (such that the expectation of any random field $\mathbb{Q}^N$ is translation-invariant), the NPCF is independent of $\vs$, and thus a function of only $(N-1)$ $D$-dimensional vectors $\vr^i$.

\subsection{Constant-Curvature Geometry}

We further assume that $\mathbb{Q}^D$ is an isotropic space of constant-curvature. In this case, the manifold permits a spatial Riemannian metric of the form
\beq\label{eq: D-dim-metric}
    d\Sigma^2_{D} = dr^2+\chi_k^2(r)\left\{d\theta_1^2+\sin^2\theta_1\left[d\theta_2^2+\sin^2\theta_2\left(d\theta_3^2+\ldots\right)\right]\right\}
\eeq
in hyperspherical coordinates $\vr \equiv \{r, \theta_1,\ldots,\theta_{D-1}\}$ for curvature parameter $k$. Here $r$ is a radial coordinate and $\theta_{i}$ are angular variables. $\chi^2_k(r)$ is defined by
\beq
    \chi_k^2(r) = \begin{cases} \frac{1}{\sqrt{k}}\sin \left(r\sqrt{k}\right), & k > 0\\ \,r, & k = 0 \\ \frac{1}{\sqrt{|k|}}\sinh \left(r\sqrt{|k|}\right), & k<0. \end{cases}
\eeq
For $D=3$, we recognize this as the constant-curvature solution to the cosmological Friedmann-Robertson-Walker equations expressed in hyperspherical coordinates with $\theta_1\equiv\theta$, $\theta_2\equiv\phi$. The sign of $k$ sets the topology of the space; $k>0$, $k=0$ and $k<0$ give the hyperbolic, flat and spherical spaces $\mathbb{H}^{D}$, $\mathbb{R}^D$ and $\mathbb{S}^D$ respectively.

A convenient basis for the constant-curvature space may be deduced by considering the eigenfunctions of the Laplace-Bertrami operator, $\Delta$, a generalization of the Laplace operator beyond $\mathbb{R}^3$. Given a metric $g_{ij}$, eigenfunctions $f(\vr)$ must satisfy
\beq
    \Delta f \equiv \frac{1}{\sqrt{|g|}}\partial_i \left(\sqrt{|g|}g^{ij}\partial_j f\right) = 0
\eeq
where $|g|$ is the metric determinant and $\partial_i$ is a partial derivative with respect to the $i$-th coordinate. Inserting \eqref{eq: D-dim-metric} leads to the partial differential equation
\beq
    \frac{1}{\chi_k^{D-1}(r)}\partial_r \left(\chi^{D-1}_k(r)\partial_r f\right) + \frac{1}{\chi_k^2(r)\sin^{D-2}\theta_1}\partial_{\theta_1}\left(\sin^{D-2}\theta_1\partial_{\theta_1}f\right)+\ldots +  \frac{1}{\chi_k^{2}(r)\sin^{2D-4}\theta_1\ldots \sin^{2}\theta_{D-2}}\partial_{\theta_{D-1}}^2f = 0
\eeq
noting that $\sqrt{|g|} = \chi_k^{D-1}(r)\sin^{D-2}\theta_1\ldots\sin\theta_{D-2}$. Assuming a separable eigenfunction $f(\vr) = R(r)Y(\hr)$, we require
\beq\label{eq: eigenfunction-eqns}
    \frac{1}{\chi_k^{D-3}(r)}\partial_r \left(\chi^{D-1}_k(r)\partial_r R(r)\right) &=& \lambda R(r)\\\nonumber
    \frac{1}{\sin^{D-2}\theta_1}\partial_{\theta_1}\left(\sin^{D-2}\theta_1\partial_{\theta_1}Y(\hr)\right)+\ldots +  \frac{1}{\sin^{2D-4}\theta_1\ldots \sin^{2}\theta_{D-2}}\partial_{\theta_{D-1}}^2Y(\hr) &=& -\lambda Y(\hr)
\eeq
for some scalar $\lambda$. The LHS of the second equation is simply equal to $\Delta_{\mathbb{S}^{D-1}}Y(\hr)$, where $\Delta_{\mathbb{S}^{D-1}}$ is the Laplace-Bertrami operator on the $(D-1)$-sphere $\mathbb{S}^{D-1}$. This may be additionally seen by noting that the metric \eqref{eq: D-dim-metric} can be written $d\Sigma^2_D = dr^2 + \chi_k^2(r)d\Omega_{D-1}^2$, where $d\Omega_{D-1}^2$ is the $(D-1)$-sphere metric. Notably, the angular solutions are \textit{independent} of the curvature parameter $k$. Physically, this corresponds to the notion that, for a homogeneous and isotropic space, spherical symmetry is respected about any given point, regardless of curvature.

\subsection{$D$-Dimensional Spherical Harmonics}

Furthermore, \eqref{eq: eigenfunction-eqns} may be written in terms of the $(D-1)$-dimensional angular momentum operator $\widehat{\bvec L}_{D-1}^2$ as
\beq
    \Delta_{\mathbb{S}^{D-1}}Y(\hr) = - \widehat{\bvec L}_{D-1}^2 Y(\hr) \equiv -\lambda Y(\hr)
\eeq
\oliver{mention that these are spherical harmonics}
The eigenfunctions of $\widehat{\bvec L}_{D-1}^2$ satisfy $\widehat{\bvec L}_{D-1}^2 Y^\ell(\hr) = \ell(\ell+D-2)Y^\ell(\hr)$ where the integer $\ell$ is a principal angular momentum quantum number. We require $(D-1)$ indices to fully specify the basis-function, $Y$, henceforth denoted as $Y^\ell_{\ell_{D-2}\ldots\ell_1}(\hr)$. 

This is the analog to the standard result $\widehat{\bvec L}_{2}^2 Y_{\ell m}(\hr) = \ell(\ell+1)Y_{\ell m}(\hr)$ in 3D space; there $\ell_1 = m$ is the spin quantum number. \oliver{give explicit forms for $D=2,3,4$?}

A general $D$-dimensional function $g(\vx)$ in a constant-curvature space can be expanded into this basis
\beq\label{eq: constant-curvature-expansion}
    g(\vr) = \sum_{\ell}\sum_{\ell_1\ldots\ell_{D-2}} g^\ell_{\ell_{D-2}\ldots\ell_1}(r)Y^\ell_{\ell_{D-2}\ldots\ell_1}(\hr)
\eeq
subject to some restrictions on $\ell_{i}$.

For $D=3$ the basis functions are straightforward:
\beq
    (D = 2) &\quad Y_\ell(\theta) = e^{i\ell \theta}\\\nonumber
    (D = 3) &\quad Y_{\ell_1\ell_2}(\theta_1,\theta_2) = P_{\ell_1}^{\ell_2}(\cos\theta_1)e^{i\ell_2\theta_2}
\eeq
where $P_\ell^m$ is the associated Legendre polynomial. Identifying $(\ell_1,\ell_2) \equiv(\ell,m)$, $(\theta_1,\theta_2)\equiv(\theta,\phi)$ we recognize the $D=3$ case as the usual spherical harmonics on the two-sphere in the Condan-Shotley phase \oliver{(true?)}.

The $D = 3$ case is just the usual spherical harmonics with $\ell_1$

\subsection{Isotropic $N$-point Basis Functions}
We now consider forming a basis for the NPCF statistic \eqref{eq: NPCF-statistic}. Firstly, we note that the NPCF exists in a space involving $(N-1)$ copies of $\mathbb{Q}^D$, and thus, by \eqref{eq: constant-curvature-expansion}, we can expand
\beq
    \zeta(\vr^1,\ldots,\vr^{N-1}) &=& \sum_{\L}\zeta_{\L}(r^1,\ldots,r^{N-1})Y^\ell_{\ell_i}(\hr^1)\ldots Y^\ell_{\ell_i}(\hr^N)
\eeq

Now, we enforce that the NPCF be invariant under rotations.
\oliver{extend to N-point basis functions here?}

\subsection{NPCF Estimator}

\beq
    \zeta_\L(r^1,\ldots,r^{N-1}) &=& \int d\vs\,\delta(\vs)\prod_{i=1}^{N-1}\int d\hr^i\,\delta(\vs+\vr^i)Y^\ell_{\ell_i}(\hr^i) \equiv \int \delta(\vs)\prod_{i=1}^{N-1}a^\ell_{\ell_i}(\vs)
\eeq
\oliver{integrals need to be in correct volume}
where
\beq
    a^\ell_{\ell_i}(\vs) &=& \int d\hr^i\,\delta(\vs+\vr^i)Y^\ell_{\ell_i}(\hr^i)
\eeq
If $\delta$ is a discrete field it can be represented as a weighted sum over $n$ Dirac delta functions:
\beq
    \delta(\vr) = \sum_{j=1}^n  w_j\,\delta_{\rm D}(\vr-\vr^j)
\eeq
for some weights $\{w_j\}$. This gives the straightforward form for the NPCF estimator:
\beq
    \zeta_\L(r^1,\ldots,r^{N-1}) &=& \sum_{j=1}^n w_j \prod_{i=1}^{N-1}a_{\ell_i}^{\ell}(\vr^j)\\\nonumber
    a^\ell_{\ell_i}(\vs) &=& \sum_{j=1}^n\,w_jY^\ell_{\ell_i}(\widehat{\vr^j-\vs})
\eeq
Each $a^{\ell}_{\ell_i}(\vs)$ function is a sum over $n$ points and must be computed at $n$ locations $\vs \in \{\vr^j\}$, thus the algorithm has complexity $\mathcal{O}(n^2)$. Furthermore, it may be applied to data on some grid \oliver{does this work in general geometries?}

\section{Applications}
\subsection{Cosmic Microwave Background}
Here we require $\mathbb{Q}^D = \mathbb{S}^2$. Parametrizing by $\vr = \theta, \phi$ where $\phi$ is a polar angle and $\theta$ a `radial' parameter on the sphere (equivalent to the angle swept out by a great circle connecting two points as viewed in the embedding space $\mathbb{R}^3$), we obtain the $D=2$ spherical harmonics:
\beq
    Y_\ell(\phi) = e^{i\ell\phi}
\eeq
whose rotational symmetry requires $\ell \in \{0,1,\ldots\} \equiv\mathbb{N}_0$. The $N$-point isotropic basis function is thus
\beq
    \P_{\ell_1\ldots\ell_N}(\phi_1,\ldots,\phi_N) = e^{i(\ell_1\phi_1+\ldots+\ell_N\phi_N)}
\eeq
with $\sum_{i=1}^N \ell_i = 0$ to ensure invariance under rotations. The 2-sphere NPCF can be expressed in this basis as
\beq
    \zeta(\vr^1,\ldots,\vr^{N-1}) &\equiv& \sum_{\ell_1+\ldots+\ell_{N-1}=0}\zeta_{\ell_1\ldots \ell_{N-1}}(\theta_1,\ldots,\theta_{N-2})e^{i\ell_1\phi_1}\ldots e^{i\ell_{N-1}\phi_{N-1}}
\eeq
with the components described by $(N-2)$ independent angular momentum numbers $\ell_i$. The estimator is given as above, with the harmonic coefficients
\beq
    a_{\ell}(\theta,\phi) = \int_{0}^{2\pi}d\phi\,e^{i\ell\phi}\delta(\vn)
\eeq
\oliver{is this true?}

\subsection{Large Scale Structure}

\subsection{Hydrodynamics}

\subsection{Other}
NB: 4D spherical harmonics represent wavefunction of hydrogen atom in mommentum space

\section{Rough}

The hyperspherical harmonics are defined as the degree $\ell_{D-1}$ homogeneous harmonic polynomials on the unit sphere $\mathbb{S}^{D-1}$
\beq\label{eq: Ylm-def}
    Y_{\vl}(\hr) &\equiv& Y_{\ell_1\ldots\ell_{D-1}}(\theta_1,\ldots,\theta_{D-1}) = \frac{1}{\sqrt{2\pi}}e^{i\ell_1\theta_1}P_{\ell_2}^{-\ell_1}(\cos\theta_2)\times \sin^{1/2}(\theta_3)P^{-(\ell_2+1/2)}_{\ell_3+1/2}(\cos\theta_3)\times\ldots\\\nonumber
    &&\,\times\,\sin^{(3-D)/2}\theta_{D-1} P^{-(\ell_{D-2}+(D-3)/2)}_{\ell_{D-1}+(D-3)/2}(\cos\theta_{D-1})\\\nonumber
    &&\,\times\,\sqrt{\frac{2\ell_2+1}{2}\frac{2\ell_3+2}{2}\ldots\frac{2\ell_{D-1}+D-2}{2}\times\frac{(\ell_2+\ell_1)!}{(\ell_2-\ell_1)!}\frac{(\ell_3+\ell_2+1)!}{(\ell_3-\ell_2)!}\ldots\frac{(\ell_{D-1}+\ell_{D-2}+D-3)!}{(\ell_{D-1}-\ell_{D-2})!}}
\eeq
where $\theta_1\in[0,2\pi)$ and $\theta_{j}\in[0,\pi)$ for $j \in \{2,\ldots,D-1\}$. Here, $P_\ell^m(x)$ are associated Legendre polynomials. Additionally $\ell_1\in\{-\ell_2,\ldots,\ell_2\}$ and  $\ell_{2}\leq\ell_3\leq\ldots\leq \ell_{D-1}$.
This is an irreducible representation of $SO(D)$ and satisfy $\Delta_{\mathbb{S}^{D-1}}Y_{\vl}(\hr) = -\ell_{D-1}(\ell_{D-1}+D-2)$. They are eigenvalues of $L_{(D-1)(D-2)}$, $L^2_{D-2}, \ldots, L^2_1$ \oliver{true}

In particular, the lowest dimensional cases give
\beq
    (D=2) & \quad Y_{\ell_1}(\theta_1) &= \frac{1}{\sqrt{2\pi}}e^{i\ell_1\theta_1}\\\nonumber
    (D=3) & \quad Y_{\ell_1\ell_2}(\theta_1,\theta_2) &= \sqrt{\frac{2\ell_2+1}{4\pi}\frac{(\ell_2+\ell_1)!}{(\ell_2-\ell_1)!}}e^{i\ell_1\theta_1}P_{\ell_2}^{-\ell_1}(\cos\theta_2)\\\nonumber
    (D=4) & \quad Y_{\ell_1\ell_2\ell_3}(\theta_1,\theta_2,\theta_3) &= \sqrt{\frac{(2\ell_2+1)(2\ell_3+2)}{8\pi}\frac{(\ell_2+\ell_1)!}{(\ell_2-\ell_1)!}\frac{(\ell_3+\ell_2+1)!}{(\ell_3-\ell_2)!}}e^{i\ell_1\theta_1}P_{\ell_2}^{-\ell_1}(\cos\theta_2)\sin^{1/2}(\theta_3)P^{-(\ell_2+1/2)}_{\ell_3+1/2}(\cos\theta_3)
\eeq
The $D=3$ case is simply the conventionally normalized spherical harmonic, made clear by identifying $(\ell_1,\ell_2)\equiv(m,\ell)$, $(\theta_1,\theta_2)\equiv(\phi,\theta)$.

Total angular momentum operator is $\widehat{\bvec L}_{D}^2 = \sum_{j<i} \widehat{L}_{ij}^2$ where $\widehat{L}_{ij} = \hat{x}_i\hat{p}_j - \hat{x}_j\hat{p}_i$ is the orbital angular momentum operator in the embedding space $\mathbb{R}^{D}$ and $i,j = 1,2,\ldots D$. The hyperspherical harmonic function satisfies $\widehat{\bvec L}^2 Y_{\vl}(\hr) = \ell_{D-1}(\ell_{D-1}+D-2)Y_{\vl}(\hr)$, \textit{i.e.} $\ell_{D-1}$ specifies the total angular momentum of the state. Furthermore, $Y_{\vl}(\hr)$ is an eigenvector of the operator $\widehat{L}_{23}$ with eigenvalue $\ell_{1}$ (which is the multidimensional analog of the spherical harmonic spin $m$), an eigenvector of $\widehat{\bvec L}_{3}^2\equiv \widehat{L}_{12}^2+\widehat{L}_{13}^2+\widehat{L}_{23}^2$ with eigenvalue $\ell_2(\ell_2+1)$, an eigenvector of $\widehat{\bvec L}_{4}^2\equiv \widehat{\bvec L}_3^2+\widehat{L}_{14}^2+\widehat{L}_{24}^2+\widehat{L}_{34}^2$ with eigenvalue $\ell_3(\ell_3+2)$, \textit{et cetera}.

The hyperspherical harmonics are orthonormal:
\beq
    \int_{\mathbb{S}^{D-1}} d\Omega_{D-1} Y_{\vl}(\hr)Y_{\vl'}^*(\hr) = \delta^{\rm K}_{\ell^{}_1\ell_1'}\ldots \delta^{\rm K}_{\ell^{}_{D-1}\ell_{D-1}'}
\eeq
with the conjugate defined via
\beq
    Y_{\ell_1\ell_2\ldots\ell_{D-1}}^*(\hr) = (-1)^{\ell_1} Y_{(-\ell_1)\ell_2\ldots\ell_{D-1}}^*(\hr),
\eeq
easily verified by \eqref{eq: Ylm-def} and the symmetries of associated Legendre polynomials.

Since the basis of hyperspherical harmonics is complete, we can expand a product of two functions of the same argument as a sum:
\beq
    Y_{\vl}(\hr)Y_{\vl'}(\hr) = \sum_{\vl''} \mathcal{G}_{\vl\,\vl'\,\vl''}Y^*_{\vl''}(\hr), \quad \mathcal{G}_{\vl\,\vl'\,\vl''} \equiv \int_{\mathbb{S}^{D-1}} d\Omega_{D-1} Y_{\vl}(\hr)Y_{\vl'}(\hr)Y_{\vl''}(\hr)
\eeq
defining $\mathcal{G}_{\vl\,\vl'\,\vl''}$ by orthonormality; this is the hyperspherical analog of the usual Gaunt integral. 

We can also consider the behavior of $Y_{\vl}(\hr)$ under rotations. Defining $R$ as a simultaneous rotation of all angular coordinates, \textit{i.e.} $\hr \to R\hr$, we may write
\beq
    Y_{\vl}(R\hr) = \sum_{\vl'} \mathcal{D}_{\vl\vl'}(R)Y_{\vl'}(\hr)
\eeq
where we have notated that the rotated state $Y_{\vl}(R\hr)$ can be written in terms of the basis functions at $\hr$ by orthonormality. The matrices $\mathcal{D}_{\vl\vl'}(R)$ are analogs of the Wigner $\mathcal{D}$-matrix in 3D-space, and are defined by
\beq
    \mathcal{D}_{\vl\,\vl'}(R) = \int_{\mathbb{S}^{D-1}}d\Omega_{D-1}Y^{}_{\vl}(\hr)Y_{\vl'}^*(R\hr)
\eeq
Since the rotation group is orthogonal, $\mathcal{D}_{\vl\,\vl'}(R)$ is unitary. Note also that $\mathcal{D}_{\vl\,\vl'}(R) \propto \delta^{\rm K}_{\ell_{D-1}^{}\ell_{D-1}'}$, since the total angular momentum is invariant under rotations.

Now consider the product states. We may form a composite state from the product of two hyperspherical harmonics as
\beq\label{eq: prod-two-states}
    P_\L(\hr^1,\hr^2) = \sum_{\vl_1\vl_2}C^\L_{\vl_1\vl_2} Y_{\vl_1}(\hr^1)Y_{\vl_2}(\hr^2)
\eeq
where the state is indexed by some set of coefficients $\L$ and $C^\L_{\vl_1\vl_2}$ are coupling coefficients. Recalling that $Y_{\vl}(\hr)$ is an eigenfunction of the $D$-dimensional angular momentum operators, we recognize this as a problem of angular-momentum addition in $D$-dimensions. In particular, given two states $\ket{\vl_1}$ and $\ket{\vl_2}$, we can form the composite state
\beq
    \ket{\vl_1,\vl_2;\vec L} = \sum_{\vl_1\vl_2}\left(\vl_1,\vl_2|\vec L\right)\ket{\vl_1}\ket{\vl_2}
\eeq
\oliver{check summation - what do we sum over - can't be everything!}, where the parentheses indicate the Clebsch-Gordan coefficient of the group $SO(D)$. This is an eigenfunction of $D$-dimensional angular momentum operators constructed from $\widehat{L}^{(1)}_{ij}+\widehat{L}^{(2)}_{ij}$ in the space $SO(D)\otimes SO(D)$.

This sets the coupling constant in \eqref{eq: prod-two-states}. \oliver{can we write this in terms of Gaunt integrals?} In general, the form of these is set by the theory of angular momentum in $D$ dimensions; see [REFS]. For $D=2,3,4$, we obtain [REFS for D=4!]
\beq
    (D=2) &\quad (\ell,\ell'|L) &= \delta^{\rm K}_{\ell+\ell',L}
    \\\nonumber
    (D=3) &\quad (\ell_1\ell_2,\ell_1'\ell_2'|L_1L_2) &= (-1)^{-\ell_2+\ell_2'-L_1}\sqrt{2L_2+1} \tj{\ell_2}{\ell_2'}{L_2}{\ell_1}{\ell_1'}{-L_1}\\\nonumber
    (D=4) &\quad (\ell_1\ell_2\ell_3,\ell_1'\ell_2'\ell_3'|L_1L_2L_3) &= (-1)^{-\ell_2+\ell_2'-L_1}(L_3+1)\sqrt{(2\ell_2+1)(2\ell_2'+1)(2L_2+1)}\tj{\ell_2}{\ell_2'}{L_2}{\ell_1}{\ell_1'}{-L_1}\begin{pmatrix}\ell_3/2 & \ell_3'/2 & L_3/2\\ \ell_3/2 & \ell_3'/2 & L_3/2 \\ \ell_2 & \ell_2' & L_2\end{pmatrix}
\eeq
The second set are the usual Clebsch-Gordan coefficients, made clearer by the identification $(\ell_1,\ell_2)=(m,\ell)$. The $3\times2$ and $3\times 3$ matrices are Wigner 3-$j$ and 9-$j$ symbols. Note that $\ell_1+\ell_1'=L_1$ is enforced in all cases (since $\ell_1$ is the eigenvector of the $\widehat{L}_{23}$ operator, which adds linearly in the combined state), and that the $D=4$ case can be written in terms of the $D=3$ Wigner 3-$j$ and 9-$j$ symbols; this occurs since $SO(4)$ is a double-cover of $SO(3)\times SO(3)$. \oliver{see e.g. \citep{biedenharn1961} and Meremianin and \citep{VanIsacker1991}}

\oliver{note what the product-states depend on}
e.g. 
\beq
    \ket{\ell_2,\ell_2';L_1,L_2} = \sum_{\ell_1\ell_1'}\left(\ell_1\ell_2,\ell_1'\ell_2'|L_1L_2\right)\ket{\ell_1\ell_2}\ket{\ell_1'\ell_2'}
\eeq


\oliver{show why the product states are invariant under rotations}


\section{Summary and Discussion}

